The Undirected Two Disjoint Shortest Paths Problem

The $k$ disjoint shortest paths problem ($k$-DSPP) on a graph with $k$ source-sink pairs $(s_i, t_i)$ asks for the existence of $k$ pairwise edge- or vertex-disjoint shortest $s_i$-$t_i$-paths. It is known to be NP-complete if $k$ is part of the input. Restricting to $2$-DSPP with strictly positive lengths, it becomes solvable in polynomial time. We extend this result by allowing zero edge lengths and give a polynomial time algorithm based on dynamic programming for $2$-DSPP on undirected graphs with non-negative edge lengths.

==> preamble.tex <==
%!TEX root=main.tex

\makeatletter

\usepackage[parfill]{parskip}
\usepackage{setspace}
\usepackage{enumitem}
\usepackage{todonotes}
\usepackage[hang,flushmargin]{footmisc}
\flushbottom

\usepackage{booktabs}

% Reihenfolge sollte eigentlich amsthm, cleveref sein. Das funktioniert bei Clara aber nicht.

\usepackage{etoolbox}

%maths

\usepackage{amsmath,amsthm,amssymb}



% graphics and figures

\usepackage{graphicx,tikz,pgfplots,float,subcaption}
\pgfplotsset{compat=1.13}
\usetikzlibrary{arrows.meta,calc,positioning}
\tikzset{%
  vertex/.style={draw=black,circle,fill=black,text width=3pt,inner sep=0pt,outer sep=1pt},%
  arc/.style={-{Latex}},%
  every label/.append style={font=\footnotesize,rectangle}%
}
\captionsetup[subfigure]{font=footnotesize,format=hang}
\patchcmd{\emailauthor}{(#2)}{}{}{}



% algorithms

\usepackage[linesnumbered,ruled]{algorithm2e}

\SetKwInput{KwParameter}{Parameter}
\SetKwInput{KwInput}{Input}
\SetKwInput{KwOutput}{Output}

% Remove line number for one line
\let\oldnl\nl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}



% references

\usepackage{hyperref}

\hypersetup{colorlinks, breaklinks}

\usepackage[noabbrev,capitalize,nameinlink]{cleveref}

\usepackage[autostyle]{csquotes}



% theorem environments

\newtheoremstyle{simple}{\parskip}{0\parskip}{\itshape}{}{\bfseries}{}{\newline}{}
\theoremstyle{simple}

\newtheorem{problem}{Problem}
\newtheorem{definition}{Definition}
\newtheorem{lemma}[definition]{Lemma}
\newtheorem{proposition}[definition]{Proposition}
\newtheorem{theorem}[definition]{Theorem}
\newtheorem{corollary}[definition]{Corollary}
\newtheorem{observation}[definition]{Observation}
\newtheorem{remark}[definition]{Remark}
\newtheorem{conjecture}[definition]{Conjecture}

\Crefname{problem}{Problem}{Problems}
\Crefname{definition}{Definition}{Definitions}
\Crefname{lemma}{Lemma}{Lemmas}
\Crefname{proposition}{Proposition}{Propositions}
\Crefname{theorem}{Theorem}{Theorems}
\Crefname{corollary}{Corollary}{Corollaries}
\Crefname{observation}{Observation}{Observations}
\Crefname{remark}{Remark}{Remarks}
\Crefname{conjecutre}{Conjecture}{Conjectures}
\Crefname{algorithm}{Algorithm}{Algorithms}

\if\@cref@capitalisetrue\else
	\crefname{problem}{problem}{problems}
	\crefname{definition}{definition}{definitions}
	\crefname{lemma}{lemma}{lemmas}
	\crefname{proposition}{proposition}{propositions}
	\crefname{theorem}{theorem}{theorems}
	\crefname{corollary}{corollary}{corollarys}
	\crefname{observation}{observation}{observations}
	\crefname{remark}{remark}{remarks}
	\crefname{conjecture}{conjecture}{conjectures}
	\crefname{algorithm}{algorithm}{algorithms}
\fi





\usepackage{xparse,mleftright}

% mathbb and mathcal

\let\Bbb\undefined

\def\mathbbfactory#1{%
	\expandafter\newcommand\csname #1bb\endcsname{\mathbb{#1}}%
}

\def\mathcalfactory#1{%
	\expandafter\newcommand\csname #1cal\endcsname{\mathcal{#1}}%
}

\newcounter{ctr}
\loop
	\stepcounter{ctr}
	\edef\X{\@Alph\c@ctr}
	\expandafter\mathbbfactory\X
	\expandafter\mathcalfactory\X
\ifnum\thectr<26
\repeat

\newcommand\zerobb{0}
\newcommand\onebb{\mathds{1}}
\newcommand\Rbbp{\Rbb_{\ge 0}}
\newcommand\Rbbpp{\Rbb_{> 0}}



% cupdots

\newcommand*{\@cupdot}[2]{%
  \ooalign{%
    $\m@th#1\cup$\cr
    \sbox0{$#1\cup$}%
    \dimen@=\ht0 %
    \sbox0{$\m@th#1\cdot$}%
    \advance\dimen@ by -\ht0 %
    \dimen@=.5\dimen@
    \hidewidth\raise\dimen@\box0\hidewidth
  }%
}

\providecommand*{\cupdot}{%
  \mathbin{%
    \mathpalette\@cupdot{}%
  }%
}

\newcommand*{\@bigcupdot}[2]{%
  \ooalign{%
    $\m@th#1\bigcup$\cr
    \sbox0{$#1\bigcup$}%
    \dimen@=\ht0 %
    \advance\dimen@ by -\dp0 %
    \sbox0{\scalebox{1.5}{$\m@th#1\cdot$}}%
    \advance\dimen@ by -\ht0 %
    \dimen@=.5\dimen@
    \hidewidth\raise\dimen@\box0\hidewidth
  }%
}

\providecommand*{\bigcupdot}{%
  \mathop{%
    \vphantom{\bigcup}%
    \mathpalette\@bigcupdot{}%
  }%
}



% harpoons

\newcommand*\@dblsty@mathpalette[2]{%
    % Works like "\mathpalette", but macro passed in #1 must take
    % (at least) three arguments, of which the first _two_ are
    % style selections.
    \mathchoice
        {#1\displaystyle       \scriptstyle       {#2}}%
        {#1\textstyle          \scriptstyle       {#2}}%
        {#1\scriptstyle        \scriptscriptstyle {#2}}%
        {#1\scriptscriptstyle  \scriptscriptstyle {#2}}%
}
\newcommand*\@dblsty@overarrow@[4]{%
    % #1 := stretchable covering arrow
    % #2 := base style
    % #3 := style for covering arrow
    % #4 := base symbol
    \vbox{\ialign{##\crcr
        #1#3\crcr
        \noalign{\nointerlineskip}%
        $\m@th\hfil #2#4\hfil$\crcr
    }}%
}

\newcommand*\leftharpoonupfill@{%
    \arrowfill@\leftharpoonup\relbar\relbar%
}

\newcommand*\rightharpoonupfill@{%
    \arrowfill@\relbar\relbar\rightharpoonup%
}

\newcommand*\overleftharp{%
    \mathpalette{\overarrow@\leftharpoonupfill@}%
}

\newcommand*\overrightharp{%
    \mathpalette{\overarrow@\rightharpoonupfill@}%
}

\newcommand*\smalloverleftharp{%
    \@dblsty@mathpalette{\@dblsty@overarrow@\leftharpoonupfill@}%
}

\newcommand*\smalloverrightharp{%
    \@dblsty@mathpalette{\@dblsty@overarrow@\rightharpoonupfill@}%
}



% paired delimiters

\NewDocumentCommand\xDeclarePairedDelimiter{mmm}
 {%
  \NewDocumentCommand#1{som}{%
   \IfNoValueTF{##2}
    {\IfBooleanTF{##1}{#2##3#3}{\mleft#2##3\mright#3}}
    {\mathopen{##2#2}##3\mathclose{##2#3}}%
  }%
 }

\xDeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\xDeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclareDocumentCommand\set{om}{\mleft\lbrace \IfNoValueF{#1}{#1 \,|\,} #2 \mright\rbrace}
\xDeclarePairedDelimiter\abs{|}{|}
\xDeclarePairedDelimiter\card{|}{|}
\xDeclarePairedDelimiter\norm{\|}{\|}



% ercs

\newcommand\textAE{\text{\AE}}
\newcommand\textae{\text{\ae}}



% problem abbreviations

\DeclareDocumentCommand\dpp{o}{\IfNoValueF{#1}{$#1$}-DPP}
\DeclareDocumentCommand\dspp{o}{\IfNoValueF{#1}{$#1$}-DSPP}
\DeclareDocumentCommand\ddspp{o}{\IfNoValueF{#1}{$#1$}-dDSPP}
\DeclareDocumentCommand\ddpp{o}{\IfNoValueF{#1}{$#1$}-dDPP}



% paths

\renewcommand\path[2]{\text{$#1$--$#2$-path}}
\newcommand\paths[2]{\text{$#1$--$#2$-paths}}
\newcommand\stpath[1]{\path{s_{#1}}{t_{#1}}}
\newcommand\stpaths[1]{\paths{s_{#1}}{t_{#1}}}



% disjoint path relations

\newcommand*{\@rightrightarrowsdot}[2]{%
  \ooalign{%
    $\m@th#1\rightrightarrows$\cr
    \sbox0{$\m@th#1\cdot$}%
    \hidewidth\box0\hidewidth
  }%
}

\providecommand*{\rightrightarrowsdot}{%
  \mathbin{%
    \mathpalette\@rightrightarrowsdot{}%
  }%
}

\providecommand*{\vertexdisjointpaths}[1]{%
  \mathbin{%
    \rightrightarrowsdot_{#1}%
  }%
}

\providecommand*{\edgedisjointpaths}[2][]{%
  \mathbin{%
    \rightrightarrows^{#1}_{#2}%
  }%
}

\providecommand*{\edgedisjointpathsop}[2][]{%
  \mathbin{%
    \rightleftarrows^{#1}_{#2}%
  }%
}

\DeclareDocumentCommand\edgedisjointshortestpath{m m}{%
  \mathbin{%
    {%
        \mathop{\rightrightarrows}%
        \limits^{\vbox to -.5\ex@{\kern-\tw@\ex@ \hbox{\scriptsize $#1$}\vss}}%
    }_{#2}%
  }%
}



\makeatother

